TempusBench: An Evaluation Framework for Time-Series Forecasting

Foundation models have transformed natural language processing and computer vision, and a rapidly growing literature on time-series foundation models (TSFMs) seeks to replicate this success in forecasting. While recent open-source models demonstrate the promise of TSFMs, the field lacks a comprehensive and community-accepted model evaluation framework. We see at least four major issues impeding progress on the development of such a framework. First, existing evaluation frameworks comprise benchmark forecasting tasks derived from often outdated datasets (e.g., M3), many of which lack clear metadata and overlap with the corpora used to pre-train TSFMs. Second, these frameworks evaluate models along a narrowly defined set of benchmark forecasting tasks, such as forecast horizon length or domain, but overlook core statistical properties such as non-stationarity and seasonality. Third, domain-specific models (e.g., XGBoost) are often compared unfairly, as existing frameworks do not enforce a systematic and consistent hyperparameter tuning convention for all models. Fourth, visualization tools for interpreting comparative performance are lacking. To address these issues, we introduce TempusBench, an open-source evaluation framework for TSFMs. TempusBench consists of 1) new datasets which are not included in existing TSFM pretraining corpora, 2) a set of novel benchmark tasks that go beyond existing ones, 3) a model evaluation pipeline with a standardized hyperparameter tuning protocol, and 4) a tensorboard-based visualization interface. We provide access to our code on GitHub: https://github.com/Smlcrm/TempusBench and maintain a live leaderboard at https://smlcrm.com/tempusbench.

==> smlcrm-logo.tex <==
\def\smlcrm@wordmark@w{862.48}
\def\smlcrm@wordmark@h{190.14}
\def\smlcrm@wordmark@draw{%
  \fill (25.41,-59.90) -- (15.06,-54.52) -- (106.12,-0.00) -- (25.41,-59.90) -- cycle;
  \fill (67.82,-81.37) -- (54.62,-74.69) -- (148.00,-21.85) -- (67.82,-81.37) -- cycle;
  \fill (110.21,-102.83) -- (94.89,-95.07) -- (189.89,-43.69) -- (110.21,-102.83) -- cycle;
  \fill (164.48,-130.24) -- (174.82,-135.62) -- (83.77,-190.14) -- (164.48,-130.24) -- cycle;
  \fill (122.07,-108.78) -- (135.27,-115.46) -- (41.88,-168.29) -- (122.07,-108.78) -- cycle;
  \fill (79.67,-87.31) -- (95.00,-95.07) -- (0.00,-146.45) -- (79.67,-87.31) -- cycle;
  \fill (253.34,-128.73) .. controls (248.32,-128.73) and (243.53,-127.96) .. (238.95,-126.43) .. controls (234.37,-124.90) and (230.77,-122.90) .. (228.14,-120.46) -- (231.62,-113.13) .. controls (234.13,-115.33) and (237.32,-117.14) .. (241.21,-118.58) .. controls (245.10,-120.02) and (249.14,-120.74) .. (253.34,-120.74) .. controls (257.16,-120.74) and (260.26,-120.30) .. (262.65,-119.42) .. controls (265.03,-118.54) and (266.79,-117.34) .. (267.91,-115.80) .. controls (269.03,-114.26) and (269.60,-112.53) .. (269.60,-110.58) .. controls (269.60,-108.32) and (268.86,-106.51) .. (267.39,-105.13) .. controls (265.92,-103.75) and (264.01,-102.64) .. (261.65,-101.79) .. controls (259.30,-100.94) and (256.71,-100.21) .. (253.89,-99.58) .. controls (251.07,-98.95) and (248.23,-98.22) .. (245.38,-97.37) .. controls (242.53,-96.52) and (239.93,-95.44) .. (237.58,-94.13) .. controls (235.23,-92.81) and (233.33,-91.04) .. (231.89,-88.82) .. controls (230.45,-86.60) and (229.73,-83.73) .. (229.73,-80.22) .. controls (229.73,-76.71) and (230.62,-73.72) .. (232.41,-70.86) .. controls (234.20,-68.01) and (236.95,-65.72) .. (240.68,-64.00) .. controls (244.41,-62.28) and (249.16,-61.41) .. (254.92,-61.41) .. controls (258.74,-61.41) and (262.54,-61.91) .. (266.30,-62.91) .. controls (270.06,-63.91) and (273.32,-65.36) .. (276.08,-67.24) -- (272.98,-74.76) .. controls (270.16,-72.88) and (267.18,-71.52) .. (264.05,-70.67) .. controls (260.91,-69.82) and (257.88,-69.40) .. (254.93,-69.40) .. controls (251.23,-69.40) and (248.19,-69.87) .. (245.81,-70.81) .. controls (243.43,-71.75) and (241.69,-73.00) .. (240.59,-74.57) .. controls (239.49,-76.14) and (238.94,-77.89) .. (238.94,-79.83) .. controls (238.94,-82.15) and (239.68,-84.00) .. (241.15,-85.38) .. controls (242.62,-86.76) and (244.54,-87.86) .. (246.89,-88.67) .. controls (249.24,-89.49) and (251.83,-90.22) .. (254.65,-90.88) .. controls (257.47,-91.54) and (260.31,-92.27) .. (263.16,-93.09) .. controls (266.01,-93.91) and (268.61,-94.97) .. (270.96,-96.29) .. controls (273.31,-97.61) and (275.21,-99.36) .. (276.65,-101.56) .. controls (278.09,-103.75) and (278.81,-106.57) .. (278.81,-110.02) .. controls (278.81,-113.47) and (277.90,-116.43) .. (276.08,-119.28) .. controls (274.26,-122.13) and (271.46,-124.42) .. (267.67,-126.14) .. controls (263.88,-127.87) and (259.10,-128.73) .. (253.33,-128.73) -- cycle;
  \fill (290.19,-127.98) -- (290.19,-62.16) -- (299.59,-62.16) -- (299.59,-127.97) -- (290.19,-127.97) -- cycle;
  \fill (313.66,-127.98) -- (313.66,-62.16) -- (321.37,-62.16) -- (350.89,-111.89) -- (346.75,-111.89) -- (375.89,-62.16) -- (383.60,-62.16) -- (383.69,-127.97) -- (374.66,-127.97) -- (374.57,-76.36) -- (376.73,-76.36) -- (350.78,-119.98) -- (346.46,-119.98) -- (320.32,-76.36) -- (322.67,-76.36) -- (322.67,-127.97) -- (313.64,-127.97) -- cycle;
  \fill (424.85,-128.73) .. controls (416.20,-128.73) and (409.40,-126.26) .. (404.45,-121.30) .. controls (399.50,-116.35) and (397.02,-109.11) .. (397.02,-99.58) -- (397.02,-62.16) -- (406.42,-62.16) -- (406.42,-99.20) .. controls (406.42,-106.53) and (408.03,-111.89) .. (411.26,-115.28) .. controls (414.49,-118.66) and (419.05,-120.36) .. (424.94,-120.36) .. controls (430.83,-120.36) and (435.48,-118.67) .. (438.71,-115.28) .. controls (441.94,-111.89) and (443.55,-106.54) .. (443.55,-99.20) -- (443.55,-62.16) -- (452.67,-62.16) -- (452.67,-99.58) .. controls (452.67,-109.11) and (450.21,-116.35) .. (445.29,-121.30) .. controls (440.37,-126.25) and (433.55,-128.73) .. (424.84,-128.73) -- cycle;
  \fill (466.09,-127.98) -- (466.09,-62.16) -- (475.49,-62.16) -- (475.49,-119.79) -- (511.12,-119.79) -- (511.12,-127.97) -- (466.09,-127.97) -- cycle;
  \fill (516.63,-127.98) -- (546.43,-62.17) -- (555.74,-62.17) -- (585.64,-127.98) -- (575.77,-127.98) -- (549.16,-67.43) -- (552.92,-67.43) -- (526.31,-127.98) -- (516.63,-127.98) -- cycle (529.32,-111.52) -- (531.86,-104.00) -- (568.90,-104.00) -- (571.63,-111.52) -- (529.32,-111.52) -- cycle;
  \fill (621.56,-128.73) .. controls (616.54,-128.73) and (611.92,-127.90) .. (607.69,-126.24) .. controls (603.46,-124.58) and (599.79,-122.23) .. (596.69,-119.19) .. controls (593.59,-116.15) and (591.16,-112.60) .. (589.40,-108.52) .. controls (587.64,-104.45) and (586.77,-99.96) .. (586.77,-95.08) .. controls (586.77,-90.20) and (587.65,-85.71) .. (589.40,-81.63) .. controls (591.15,-77.56) and (593.60,-74.00) .. (596.73,-70.96) .. controls (599.86,-67.92) and (603.55,-65.57) .. (607.78,-63.91) .. controls (612.01,-62.25) and (616.63,-61.42) .. (621.65,-61.42) .. controls (626.67,-61.42) and (631.41,-62.28) .. (635.71,-64.01) .. controls (640.00,-65.73) and (643.65,-68.29) .. (646.66,-71.67) -- (640.55,-77.59) .. controls (638.04,-74.96) and (635.22,-73.00) .. (632.09,-71.71) .. controls (628.96,-70.43) and (625.60,-69.78) .. (622.03,-69.78) .. controls (618.46,-69.78) and (614.90,-70.41) .. (611.74,-71.66) .. controls (608.57,-72.91) and (605.83,-74.67) .. (603.51,-76.92) .. controls (601.19,-79.18) and (599.39,-81.86) .. (598.10,-84.96) .. controls (596.82,-88.06) and (596.17,-91.43) .. (596.17,-95.07) .. controls (596.17,-98.71) and (596.81,-102.07) .. (598.10,-105.18) .. controls (599.38,-108.28) and (601.19,-110.96) .. (603.51,-113.22) .. controls (605.83,-115.48) and (608.57,-117.23) .. (611.74,-118.48) .. controls (614.90,-119.74) and (618.33,-120.36) .. (622.03,-120.36) .. controls (625.73,-120.36) and (628.96,-119.72) .. (632.09,-118.43) .. controls (635.22,-117.15) and (638.04,-115.16) .. (640.55,-112.46) -- (646.66,-118.38) .. controls (643.65,-121.77) and (640.00,-124.34) .. (635.71,-126.09) .. controls (631.41,-127.85) and (626.70,-128.72) .. (621.56,-128.72) -- cycle;
  \fill (657.75,-127.98) -- (657.75,-62.16) -- (683.42,-62.16) .. controls (689.18,-62.16) and (694.10,-63.07) .. (698.18,-64.89) .. controls (702.25,-66.71) and (705.39,-69.34) .. (707.58,-72.79) .. controls (709.77,-76.24) and (710.87,-80.34) .. (710.87,-85.10) .. controls (710.87,-89.86) and (709.77,-93.95) .. (707.58,-97.37) .. controls (705.39,-100.79) and (702.25,-103.40) .. (698.18,-105.22) .. controls (694.10,-107.04) and (689.18,-107.95) .. (683.42,-107.95) -- (662.92,-107.95) -- (667.15,-103.62) -- (667.15,-127.97) -- (657.75,-127.97) -- cycle (667.15,-104.57) -- (662.92,-99.96) -- (683.13,-99.96) .. controls (689.15,-99.96) and (693.71,-98.66) .. (696.81,-96.06) .. controls (699.91,-93.46) and (701.46,-89.81) .. (701.46,-85.11) .. controls (701.46,-80.41) and (699.91,-76.78) .. (696.81,-74.20) .. controls (693.71,-71.63) and (689.15,-70.35) .. (683.13,-70.35) -- (662.92,-70.35) -- (667.15,-65.65) -- (667.15,-104.57) -- cycle (701.75,-127.98) -- (685.02,-104.10) -- (695.08,-104.10) -- (712.00,-127.98) -- (701.75,-127.98) -- cycle;
  \fill (751.01,-128.73) .. controls (742.36,-128.73) and (735.56,-126.26) .. (730.61,-121.30) .. controls (725.66,-116.35) and (723.18,-109.11) .. (723.18,-99.58) -- (723.18,-62.16) -- (732.58,-62.16) -- (732.58,-99.20) .. controls (732.58,-106.53) and (734.19,-111.89) .. (737.42,-115.28) .. controls (740.65,-118.66) and (745.21,-120.36) .. (751.10,-120.36) .. controls (756.99,-120.36) and (761.64,-118.67) .. (764.87,-115.28) .. controls (768.10,-111.89) and (769.71,-106.54) .. (769.71,-99.20) -- (769.71,-62.16) -- (778.83,-62.16) -- (778.83,-99.58) .. controls (778.83,-109.11) and (776.37,-116.35) .. (771.45,-121.30) .. controls (766.53,-126.25) and (759.71,-128.73) .. (751.00,-128.73) -- cycle;
  \fill (792.43,-127.98) -- (792.43,-62.16) -- (800.14,-62.16) -- (829.66,-111.89) -- (825.52,-111.89) -- (854.66,-62.16) -- (862.37,-62.16) -- (862.46,-127.97) -- (853.43,-127.97) -- (853.34,-76.36) -- (855.50,-76.36) -- (829.55,-119.98) -- (825.23,-119.98) -- (799.09,-76.36) -- (801.44,-76.36) -- (801.44,-127.97) -- (792.41,-127.97) -- cycle;
}
\def\smlcrm@emblem@w{531.22}
\def\smlcrm@emblem@h{531.93}
\def\smlcrm@emblem@draw{%
  \fill (71.08,-167.57) -- (42.14,-152.52) -- (296.87,-0.00) -- (71.08,-167.57) -- cycle;
  \fill (189.72,-227.62) -- (152.80,-208.94) -- (414.04,-61.12) -- (189.72,-227.62) -- cycle;
  \fill (308.32,-287.67) -- (265.45,-265.96) -- (531.22,-122.23) -- (308.32,-287.67) -- cycle;
  \fill (460.14,-364.37) -- (489.08,-379.41) -- (234.35,-531.93) -- (460.14,-364.37) -- cycle;
  \fill (341.50,-304.31) -- (378.41,-323.00) -- (117.17,-470.81) -- (341.50,-304.31) -- cycle;
  \fill (222.89,-244.27) -- (265.76,-265.97) -- (0.00,-409.70) -- (222.89,-244.27) -- cycle;
}

